Study of charmonium production using decays to hadronic final states with the LHCb experiment

Studies of charmonium properties and production mechanism started with the discovery of $J/\psi$ meson. Since more than 40 years the charmonium production mechanism is still not entirely understood. Following the era of investigations at $e^+e^-$ machines, nowadays, charmonium states are copiously produced at hadron colliders, that allows systematic studies of their resonance parameters, production observables and decays. Despite large production rates, many charmonium states are barely studied due to the complications of their reconstruction against a large background level. The LHCb experiment provides a unique opportunity to study S-wave and P-wave charmonium states using their decays to hadrons. This allows measuring production observables of $\eta_c$ and $\chi_c$ charmonium states. According to the theoretical formalism of Non-Relativistic QCD (NRQCD), the production observables of the same wave charmonium states are linked. Hence, the LHCb measurements provide a series of stringent tests of NRQCD. In the framework of this thesis, the first measurement of the $\eta_c(1S)$ differential production cross-section at $\sqrt{s}=13\,TeV$ and the most precise to date single mass measurement are performed, where the $\eta_c(1S)$ state is reconstructed via its decay to $p\bar{p}$. In addition, the production of the $\chi_c$ and $\eta_c(2S)$ states in $b$-hadron decays is studied using decays to $\phi\phi$. The obtained results are confronted with existing theory predictions. The original phenomenological analysis concludes that the description of charmonium prompt production and production in inclusive $b$-hadron decays in an entire range of transverse momentum remains a challenge.

==> Conclusions.tex <==
\section*{Conclusions}
This thesis presents new developed methods and studies done for the ILC project.
Detectors at the ILC are designed for the application of Particle Flow algorithms, which enhance the physics performance by using the information from the highly granular calorimeters. 

The high granular \ecalp\ was constructed and tested by the CALICE collaboration. 
During this thesis, a track-finding algorithm was developed allowing to reconstruct secondary tracks emerged from hadronic interactions in the \ecalp.
The \ecalp\ simulation was compared to the data using the new observables from the track-finding algorithm. 
All tested simulation models shows a good performance in terms of the new observables. 
These results have been accepted as CALICE Preliminary results and were presented at the Vienna Conference on Instrumentation (VCI) and the IEEE Nuclear Science Symposium.
The developed track-finding algorithm can be applied for the Particle Flow reconstruction or at least for its validation in simplified scenarios.

In this thesis, the b-quark charge technique is used for reconstruction of top and bottom quark polar angle distribution.
The developed methods are applied in two channels, $e^+e^-\to t\bar{t}$ and $e^+e^-\to b\bar{b}$ processes at $\sqrt{s} = 500$\,GeV and 250\,GeV, respectively.

The developed b-quark charge reconstruction technique uses information from reconstructed secondary and tertiary vertices. 
Using the standard reconstruction algorithm one has a low b-quark charge purity of 66\%.
It was found, that missing particles from the secondary and tertiary vertices degrade the b-quark charge purity. 
%A detailed study was made to establish the reasons behind the missing particles. 
To increase the purity of the b-quark charge, the developed Vertex Charge Recovery algorithm adds the missing particles to the reconstructed vertices and, as a result, it increases the b-quark charge purity by 7\%.
The kaons from the secondary or tertiary vertices deliver information about the initial quark charge. 
To increase the kaon identification efficiency, an angular correction was applied to the reconstructed $dE/dx$ values. 
After correction one has 97\% purity and 87\% efficiency of the kaon identification.

The top quark polar angle is reconstructed in the semileptonic channel using a combination of the b-quark charge with the $W^\pm$ lepton charge. 
This technique improves the reconstruction efficiency by 25\% as comparing to the previous result~\cite{bib:ILCTOP}.
Moreover, the b-quark charge technique can be applied in the fully hadronic \ttbar\ pair decays, which should increase significantly the available statistics to determine the top quark electroweak couplings. 

This thesis addresses the topic of \bbbar\ pair production, which have never been studied using the ILC environment. 
This study is motivated by the $A_{FB}$ measurement at $Z^0$ pole by LEP collaborations, which disagrees by 2.5 standard deviations from the \sm\ prediction.
This deviation shifts the right-handed $Z^0b\bar{b}$ coupling by 25\% with 10\% uncertainty.
The b-quark charge measurement is the only possible method to compute the b-quark polar angle distribution. 
Two major problems were discovered: the event migration and the forward region efficiency decrease. 
It was found, that residual charge impurity contaminates completely the backward region of b-quark polar angle distribution for the left-handed beam configuration.
The procedure of the data-driven charge purity measurement allows to correct the distribution for residual contamination. 
As the result, the reconstructed b-quark polar angle is usable for the extraction of electroweak couplings and form factors of the b-quark. 
Given the accuracy predicted at ILC on the right-handed coupling, 5 times better then at LEP, the LEP anomaly will be either fully confirmed or definitely discarded. 
A paper publication based on this work is on-going.
In view of the observed experimental shortcomings reported in this thesis, the ILD collaboration initiated an optimization of the forward region detectors design to address the forward region inefficiency problem.

%The b-quark charge measurement requires an ultimate performance from all subdetectors and all reconstruction algorithms. 
%The Particle Flow reconstruction scheme is essential for the b-jet charge technique.


==> Cover_PHENIICS/title.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Modèle pour  1ère de couverture des thèses préparées à l'Université Paris-Saclay, basé sur le modèle produit par Guillaume BRIGOT / Template for back cover of thesis made at Université Paris-Saclay, based on the template made by Guillaume BRIGOT
% %%% Mis à jour par Aurélien ARNOUX (École polytechnique)/ Updated by Aurélien ARNOUX (École polytechnique)
% %%% Les instructions concernant chaque donnée à remplir sont données en bloc de commentaire / Rules to fill this file are given in comment blocks
% %%% ATTENTION Ces informations doivent tenir sur une seule page une fois compilées / WARNING These informations must contain in no more than one page once compiled
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Version du 19 juillet 2018 (Merci à Hadrien VROYLANDT (Univ. Paris-Sud) pour ses suggestions et corrections)
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \documentclass[a4paper]{article}
% \usepackage[utf8]{inputenc}
% \usepackage{helvet}
% \renewcommand{\familydefault}{\sfdefault}
% \usepackage{geometry}
% \geometry{
% 	left=16mm,
% 	top=30mm,
% 	right=16mm,
% 	bottom=30mm
% }
% \usepackage{xcolor}
% \definecolor{bordeau}{rgb}{0.3515625,0,0.234375}
% \usepackage[absolute,overlay]{textpos}
% \usepackage{graphicx}
% \usepackage{lipsum}
% \usepackage{hyperref}
% \usepackage{array}
% \usepackage{caption}
% \usepackage{multicol}
% \setlength{\columnseprule}{0pt}
% \setlength\columnsep{10pt}
% \usepackage[french]{babel}

% \label{form}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Formulaire / Form
% %%% Remplacer les paramètres des \newcommand par les informations demandées / Replace \newcommand parameters by asked informations
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newcommand{\PhDTitle}{Study of charmonium production using decays to hadronic final states with the LHCb experiment} 

% \newcommand{\PhDTitleFRR}{\normalsize \'{E}tudes de production des \'{e}tats de charmonium avec leurs d\'{e}sint\'{e}grations vers des hadrons dans l'exp\'{e}rience LHCb}
% %% Titre de la thèse / Thesis title
% \newcommand{\PhDname}{Andrii Usachov} 															%% Civilité, nom et prénom /  Civility, first name and name 
% \newcommand{\NNT}{2019SACLS135} 															%% Numéro National de Thèse (donnée par la bibliothèque à la suite du 1er dépôt)/ National Thesis Number (given by the Library after the first deposit)

% \newcommand{\ecodoctitle}{Particules, Hadrons, Énergie, Noyau, Instrumentation, Imagerie, Cosmos et Simulation} 													%% Nom de l'ED. Voir site de l'Université Paris-Saclay / Full name of Doctoral School. See Université Paris-Saclay website
% \newcommand{\ecodocacro}{PHENIICS}																%% Sigle de l'ED. Voir site de l'Université Paris-Saclay / Acronym of the Doctoral School. See Université Paris-Saclay website
% \newcommand{\ecodocnum}{576} 																%% Numéro de l'école doctorale / Doctoral School number
% \newcommand{\PhDspeciality}{Physique des particules} 										%% Spécialité de doctorat / Speciality 
% \newcommand{\PhDworkingplace}{l'Université Paris-Sud} 
% \newcommand{\PhDlab}{Laboratoire de l'accélérateur linéaire}										%% Établissement de préparation / PhD working place : l'Université Paris-Sud, l'Université de Versailles-Saint-Quentin-en-Yvelines, l'Université d'Evry-Val-d'Essonne, l'Institut des sciences et industries du vivant et de l'environnement (AgroParisTech), CentraleSupélec,l'Ecole normale supérieure de Cachan, l'Ecole Polytechnique, l'Ecole nationale supérieure de techniques avancées, l'Ecole nationale de la statistique et de l’administration économique, HEC Paris, l'Institut d'optique théorique et appliquée, Télécom ParisTech, Télécom SudParis   
% \newcommand{\defenseplace}{Orsay} 											%% Ville de soutenance / Place of defense
% \newcommand{\defensedate}{05 Juillet 2019} 															%% Date de soutenance / Date of defense

% %%% Établissement / Institution
% %%% Si la thèse a été produite dans le cadre d'une co-tutelle, commenter la partie "Pas de co-tutelle" et décommenter la partie "Co-tutelle" / If the thesis has been prepared in guardianship, comment the part "Pas de co-tutelle" and uncomment the part "Co-tutelle"

% 	%%%%%%%%%%%%%%%%%%%%%%%%%
% 	%%% Pas de co-tutelle %%%
% 	%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\logoEtt}{blank}																%% NE PAS MODIFIER / DO NOT MODIFY
% \newcommand{\vpostt}{0.1} 																	%% NE PAS MODIFIER / DO NOT MODIFY
% \newcommand{\hpostt}{6}																		%% NE PAS MODIFIER / DO NOT MODIFY
% \newcommand{\logoEt}{UPSUD} 																	%% Logo de l'établissement de soutenance. Indiquer le sigle / Institution logo. Indicate the acronym : AGRO, CENTSUP, ENS, ENSAE, ENSTA, HEC, IOGS, TPT, TSP, UEVE, UPSUD, UVSQ, X 
% \newcommand{\vpos}{0.15}																		%% À modifier au besoin pour aligner le logo verticalement / If needed, modify to align logo vertilcally
% \newcommand{\hpos}{11}																		%% À modifier au besoin pour aligner le logo horizontalement / If needed, modify to align logo horizontaly

% 		%%%%%%%%%%%%%%%%%%
% 		%%% Co-tutelle %%%
% 		%%%%%%%%%%%%%%%%%%

% % \newcommand{\logoEt}{etab} 																%% Logo de l'université partenaire. Placer le fichier .png dans le répertoire '/media/etab' et indiquer le nom du fichier sans l'extension / Logo of partner university. Place the .png file in the directory '/media/etab' and point the file name without the extension
% % \newcommand{\vpos}{0.1}																	%% À modifier au besoin pour aligner les logos verticalement / If needed, modify to align logos vertilcally
% % \newcommand{\hpos}{11}																		%% À modifier au besoin pour aligner les logos horizontalement / If needed, modify to align logos horizontaly
% % \newcommand{\logoEtt}{etab2}  																%% Logo de l'établissement de soutenance. Le nom du fichier correspond au sigle de l'établissement /  Institution logo. Filename correspond to institution acronym : AGRO, CENTSUP, ENS, ENSAE, ENSTA, HEC, IOGS, TPT, TSP, UEVE, UPSUD, UVSQ, X 
% % \newcommand{\vpostt}{0.1} 																	%% À modifier au besoin pour aligner les logos verticalement / If needed, modify to align logos vertilcally
% % \newcommand{\hpostt}{6}																	%% À modifier au besoin pour aligner les logos horizontalement / If needed, modify to align logos horizontaly


% %%% JURY

% % Lors du premier dépôt de la thèse le nom du président nest pas connu, le choix du président se fait par les membres du Jury juste avant la soutenance. La précision est apportée sur la couverture lors du second dépôt / Choice of the jury's president is made during the defense. Thus, it must be specified only for the second file deposition in ADUM.
% % Tous les membres du juty listés doivent avoir été présents lors de la soutenance / All the jury members listed here must have been present during the defense.

% %%% Membre n°1 (Président) / Member n°1 (President)
% \newcommand{\jurynameA}{Fabien Cavalier}
% \newcommand{\juryadressA}{Directeur de recherche (LAL)}
% \newcommand{\juryroleA}{Président}

% %%% Membre n°2 (Rapporteur) / Member n°2 (President)
% \newcommand{\jurynameB}{Claudia Patrignani}
% \newcommand{\juryadressB}{Professor (University of Bologna)}
% \newcommand{\juryroleB}{Rapportrice}

% %%% Membre n°3 (Rapporteur) / Member n°3 (President)
% \newcommand{\jurynameC}{Antonio Vairo}
% \newcommand{\juryadressC}{Professor (Technical University of Munich)}
% \newcommand{\juryroleC}{Rapporteur}

% %%% Membre n°4 (Examinateur) / Member n°4 (President)
% \newcommand{\jurynameD}{Vincenzo Vagnoni}
% \newcommand{\juryadressD}{Professor (INFN, Bologna)}
% \newcommand{\juryroleD}{Examinateur}

% %%% Membre n°5 (Directeur de thèse) / Member n°5 (Thesis supervisor)
% \newcommand{\jurynameE}{Tatsuya Nakada}
% \newcommand{\juryadressE}{Professor (EPFL, Lausanne)}
% \newcommand{\juryroleE}{Examinateur}

% %%% Membre n°7 (Invité) / Member n°7 (Guest)
% \newcommand{\jurynameF}{Achille Stocchi}
% \newcommand{\juryadressF}{Professeur (LAL)}
% \newcommand{\juryroleF}{Examinateur}

% %%% Membre n°6 (Co-directeur de thèse) / Member n°6 (Thesis co-supervisor)
% \newcommand{\jurynameG}{Sergey Barsuk}
% \newcommand{\juryadressG}{Directeur de recherche (LAL)}
% \newcommand{\juryroleG}{Directeur de th\`{e}se}

% % %%% Membre n°7 (Invité) / Member n°7 (Guest)
% % \newcommand{\jurynameG}{Achille Stocchi}
% % \newcommand{\juryadressG}{Professeur}
% % \newcommand{\juryroleG}{Examinateur}

% % %%% Membre n°8 (Invité) / Member n°8 (Guest)
% % \newcommand{\jurynameH}{Prénom Nom}
% % \newcommand{\juryadressH}{Statut, Établissement (Unité de recherche)}
% % \newcommand{\juryroleH}{Invité}

% %% Il est possible d'ajouter des membres supplémentaires selon le même modèle / More jury members can be added according to the same model

% \label{layout}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Mise en page / Page layout      
% %%% NE RIEN MODIFIER EXCEPTÉ LA PARTIE CONCERNANT LE JURY (voir \label{jury}) SI BESOIN / DO NOT MODIFY EXCEPT SECTION CONCERNING JURY (see \label{jury}) IF NEEDED
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Méta-données du PDF / PDF meta-datas
% \hypersetup{
% 	pdfauthor={\PhDname},
% 	pdfsubject={Manuscrit de thèse de doctorat},
% 	pdftitle={\PhDTitle},
% }

% \begin{document}


% \thispagestyle{empty}

% %\color{bordeau} \hfill \vfill \tiny \ecodocnum
% \begin{textblock}{5}(0,0)
% 	\textblockcolour{bordeau}
% 	%\vspace{10mm}
% 	\includegraphics [scale=1]{media/bande.png}
% 	\vspace{300mm}
% \end{textblock}

% \begin{textblock}{1}(0.6,9.5)
	
% 	\Huge{\rotatebox{90}{\color{white}{\fontsize{38}{54}\selectfont Thèse de doctorat}}}
% \end{textblock}

% \begin{textblock}{1}(0.6,3)
% 	\Large{\rotatebox{90}{\color{white}{NNT : \NNT}}}
% \end{textblock}


                            

% % \begin{textblock}{1}(\hpostt,\vpostt)
% % 	\textblockcolour{white}
% % 	\includegraphics[scale=1]{media/etab/\logoEtt.png}
% % \end{textblock}

% \begin{textblock}{1}(\hpos,\vpos)
% 	\textblockcolour{white}
% 		\includegraphics[scale=1]{media/\logoEt.png}	
% \end{textblock}

% % \begin{textblock}{1}(\hpos,\vpos)
% % 	\textblockcolour{white}
% % 		\includegraphics[scale=0.35]{media/logo_ups.eps}	
% % \end{textblock}

% %\vspace{6cm}
% %% Texte
% \begin{textblock}{10.}(5.7,3)
% 	\textblockcolour{white}
	
% 	\color{bordeau}
% 	%\begin{center}  
% 	\begin{flushright}%\huge
% 		\fontsize{30}{36}\selectfont{\PhDTitle} \bigskip %% Titre de la thèse 
% 		\vfill
% 		\large \textbf{\PhDTitleFRR} \\ \bigskip
% 		\color{black} %% Couleur noire du reste du texte
% 		\normalsize {Thèse de doctorat de l'Université Paris-Saclay} \\
% 		préparée à \PhDworkingplace \\
% 		\PhDlab \\ \bigskip
% 		\vfill
% 		Ecole doctorale n$^{\circ}$\ecodocnum ~\ecodoctitle ~(\ecodocacro)  \\
		
% 		\small{Spécialité de doctorat: \PhDspeciality} \bigskip %% Spécialité 
% 		\vfill  
% 		\footnotesize{Thèse présentée et soutenue à \defenseplace, le \defensedate, par} \bigskip
% 		\vfill
% 		\Large{\textbf{\textsc{\PhDname}}} %% Nom du docteur
% 		\vfill
% 		%\bigskip
% 	\end{flushright}
	
% 	%\end{center}
% 	\color{black}
% 	%% Jury
% 	\begin{flushleft}
		
% 		\small Composition du Jury :
% 	\end{flushleft}
% 	%% Members of the jury

% 	\small
% 	%\begin{center}
% 	\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% 	\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}lm{#1}}
	
% 	\label{jury} 																				%% Mettre à jour si des membres ont été ajoutés ou retirés / Update if members have been added or removed
% 	\begin{flushleft}
% 	\begin{tabular}{@{} L{9.0cm} R{4.5cm}}
% 		\jurynameA  \\ \juryadressA & \juryroleA \\[5pt]
% 		\jurynameB  \\ \juryadressB & \juryroleB \\[5pt]
% 		\jurynameC  \\ \juryadressC & \juryroleC \\[5pt]
% 		\jurynameD  \\ \juryadressD & \juryroleD \\[5pt]
% 		\jurynameE  \\ \juryadressE & \juryroleE \\[5pt]
% 		\jurynameF  \\ \juryadressF & \juryroleF \\[5pt]
% 		\jurynameG  \\ \juryadressG & \juryroleG \\[5pt]
% 		%\jurynameH  \\ \juryadressH & \juryroleH \\[5pt]
% 	\end{tabular} 
% 	\end{flushleft}   
% 	%\end{center}
% \end{textblock}


% \begin{textblock}{0.}(12,15)
% 	\Large{\rotatebox{0}{\color{black}{LAL 19-014}}}
% \end{textblock}


% \end{document}
% \newpage
% \setcounter{page}{2}
% \mbox{~}

% \cleardoublepage

==> Francais.tex <==
\section{R\'esum\'e en fran\c cais}

\renewcommand{\sm}{modèle standard}
\renewcommand{\bsm}{au delà du modèle standard}
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\subsection*{Introduction}


L'International Linear Collider \cite{bib:ILC} (ILC) est un projet de collisionneur électron-positon à haute énergie destiné à la recherche de la nouvelle physique par des mesures de précision.
%L'ILC est conçu pour fonctionner à l'énergie centrale de masse $\sqrt{s} = 500$\gev, ce qui est idéal pour des études sur les interactions électriques du quark top.
%L'état initial leptonique bien connu à l'ILC permet une analyse propre, indépendante du modèle des processus Modele Standard ainsi que des recherches des nouvelles particules.
L’énergie dans le centre de masse peut être variée entre la masse du boson $Z^0$ et 1\,TeV couvrant ainsi les masses de toutes les particules du modèle standard. 
La Figure~\ref{fig:ILCSchemeF} représente une vue synoptique du complexe de l’accélérateur et de ses dimensions. 
L’état initial des collisions est composé par des particules élémentaires ce qui conduit à une excellente contrôle des erreurs théoriques et constitue donc une situation idéale pour des mesures de précision. 
Le programme scientifique de l'ILC porte sur une étude profonde du boson de Higgs ainsi que sur la détermination des couplages électrofaibles des fermions; notamment ceux des quarks lourds bottom et top. Le potentiel de physique sera renforcé par des faisceaux polarisés où dans la suite $P_{e-}$ représente la polarisation du faisceau d’electrons et $P_{e+}$ représente celle du faisceau de positons.

%La vue schématique du système d'accélération complète est présentée dans la Figure~\ref {fig:ILCSchemeF}.

%Le potentiel de physique du projet de l'ILC sera renforcé par des faisceaux polarisés, qui peuvent être utilisés pour supprimer les processus en bruit de fond de la physique électrofaible.

\begin{figure}
	{\centering
		\protect\includegraphics[width=0.95\textwidth]{graphics/ILC_scheme.jpg}
		\caption{\sl Vue sch\'ematique de l'ILC.}
		\label{fig:ILCSchemeF}
	}
\end{figure}

L’ILC devrait avoir deux d\'etecteurs, SiD et ILD, qui vont fonctionner de mani\`ere alternative.
% pour assurer la v\'erification des r\'esultats.
Cette thèse est concentre sur l'expérience ILD. 

ILD (International Large Detector) est un concept pour un détecteur multi-tâches de haute précision. %, conçu pour atteindre les objectifs de physique de l'ILC~\cite{Behnke:2013lya}.
%La vue schématique de l'ILD est présentée dans la Figure~\ref {fig:ILCSchemeF}.
Comme montr\'e dans la vue schématique, Fig.~\ref {fig:ILDSchemeF}, ILD est compos\'e de plusieurs sous-d\'etecteurs concentriques:
\begin{itemize}
	\item un d\'etecteur de vertex à pixel multicouche (VTX), avec les disques trajectométriques vers l'avant (FTD);
	%\item le large de la tube de faisceau la trajectométrie est completée par un système des disques avec des pixels et des bandes de silicium;
	\item deux cylindres de silicium (SIT);
	\item une ”Time Projection Chamber” (TPC) comme d\'etecteur de traces central;
	\item un calorim\`etre \'electromagn\'etique hautement granulaire (ECAL);
	\item un calorim\`etre hadronique hautement granulaire (HCAL);
	\item une bobine supraconductrice, qui cr\'ee un champ magn\'etique axial de 3.5~Tesla.
	\item un d\'etecteur pour les muons et les fins de cascades hadroniques (TCMT).
\end{itemize}

\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\protect\includegraphics[width=0.95\textwidth]{graphics/ILD.png}
		
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=0.9\textwidth]{graphics/ILDtracking.png}
		
	\end{subfigure}
	\caption{\sl Gauche: Vue sch\'ematique d'un quadrant de l'ILD. Droite: Gros plan sur les détecteurs internes.}
	\label{fig:ILDSchemeF}
\end{figure}
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{Calorim\`etre \'electromagn\'etique silicium-tungst\`ene hautement granulaire}

Un calorim\`etre \'electromagn\'etique de silicium tungst\`ene (SiW-ECAL) est le
choix favorisé d'ILD.

La collaboration CALICE (CAlorimetry for the LInear Collider Experiments) a construit et testé un prototype SiW-ECAL dont la vue schématique du prototype est présentée dans la Figure~\ref {fig:ECAL-schemeF}.

L'avantage du tungstène est sa grande longueur d'interaction ($\lambda_I = 96$\,mm), compar\'ee \`a sa longueur de radiation  $X_0 = 3.5$\,mm. Cela permet une bonne s\'eparation longitudinale entre les photons et les hadrons. 
Des capteurs de silicium sous-divisés en pixels d'une taille de $1\times1$\,cm$^2$ servent comme mat\'eriau actif. 
\begin{figure}
	\centering
	\protect\includegraphics[width=0.55\textwidth]{ECAL/graphics/ecal-new.png}
	\caption{\label{fig:ECAL-schemeF} \sl  Vue sch\'ematique du \ecal.}
\end{figure}

Cette thèse présente une analyse de données enregistrées avec le prototype SiW-ECAL lors d'un campagne de test en faisceau au FNAL (Etats-Unis) en 2008.  
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{L'algorithme de reconstruction de traces}
L'objectif principal de l'algorithme de traces developpé pour cette thèse est la détection de traces diffusées vers l'avant qui proviennent de l'interaction entre les pions primaires et le matériau absorbant en l'absence d'un champ magnétique.

Le schéma d'exécution de l'algorithme est comme suit:
%L'algorithme suit le sch\'ema d'ex\'ecution suivant:
\begin{itemize}
	\item La région d'interaction est identifiée par un critère topologique et séparée pour une analyse plus approfondie, voir Fig.~\ref{fig:testF};
	\item Les dépôts d'énergie restants sont regroupés dans des amas de pixels appelés  clusters dans la suite, voir Fig.~\ref{fig:democlusterF};
	\item Les clusters obtenus sont classés pour séparer ceux qui ressemblent aux traces des signaux provenants du bruit résiduel; 
	\item Après la classification, les clusters qui appartiennent à la même particule secondaire   sont fusionnés en une seule trace.
	
\end{itemize}
\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/graphics/before.png}
		\caption{\label{fig:beforeF} \sl avec région d'interaction.}
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/graphics/after2.png}
		\caption{\label{fig:afterF} \sl sans région d'interaction.}
	\end{subfigure}
	\caption{ \sl Visualisation de l'interaction d'un pion primaire 10\,GeV d'\'energie enregistrée au FNAL 2008 avant \textit{(a)} et apr\'es suppression de la région d'interaction\textit{(b)}. }
	%Event 16-17 in Data10.root
	\label{fig:testF}
\end{figure}


\begin{figure}
	\centering
	\protect\includegraphics[width=0.55\textwidth]{ECAL/graphics/demo-v3.pdf}
	\caption{\label{fig:democlusterF} \sl Illustration des étapes de la clusterisation. Les pixels actives sont représentés par des cubes bleus, et la zone de recherche pour des signaux contigus est indiquée par des cubes rouges. Les flèches bleues indiquent la direction du flux de clusterisation.}
\end{figure}

%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{Comparaison des simulations et des données réelles}
La figure \ref{fig:irexampleF} montre les distributions du rapport entre l'énergie déposée dans la zone d'interaction et l'énergie totale dans le détecteur. Les données sont comparées aux prédictions de trois modèles de simulation des gerbes hadroniques proposés par le logiciel GEANT4.  
%La figure \ref{fig:irexampleF} montre les comparaisons des distributions d'énergie de la région d'interaction sur le dépôt d'énergie total $f_ {IR}$ entre les données et les trois listes de physique de {\sc Geant4}.
La première case de chaque histogramme totalise les événements pour lesquels aucune région d'interaction n'est trouvée par l'algorithme.


\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/e-ir-2.pdf}
		\caption{\label{fig:efr2F} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/e-ir-10.pdf}
		\caption{\label{fig:efr10F} }
	\end{subfigure}
	\caption{\label{fig:irexampleF} \sl% {\bf Fig.~\ref{fig:efr2}: Remind me how the linear plot looks like} 
		Comparaison de $f_{IR}$ entre les données et les simulations pour trois listes {\sc Geant}4 physiques pour 2 GeV (a) et 10 GeV (b) d'énergie de la particule primordiale.}
\end{figure}

Dans la figure \ref{fig:irgraphF} la valeur moyenne de $f_ {IR}$ est présentée en fonction de l'énergie du faisceau.% pour les énergies du faisceau de 2, 4, 6, 8 et 10 \, GeV.
La valeur moyenne de $f_{IR}$ prédit par les modèles de simulation est jusqu'à 20\% inférieure à celle observée dans les données.

\begin{figure}
	\centering
	\protect\includegraphics[width=0.5\textwidth]{ECAL/plots/e-ir-graph.pdf}
	\caption{\label{fig:irgraphF} \sl  Fraction moyenne du dépôt d'énergie dans la région d'interaction pour les données et les simulations  pour trois modèles de simulation proposés par le logiciel \geant\ en fonction de l'énergie du faisceau (2\,GeV à 10\,GeV).}
\end{figure}

%\begin{figure}
%	\centering
%	\begin{subfigure}{0.5\textwidth}
%		\centering
%		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/r-ir-2.pdf}
%		\caption{\label{fig:rir2F} }
%	\end{subfigure}% 
%	\begin{subfigure}{0.5\textwidth}
%		\centering
%		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/r-ir-10.pdf}
%	\end{subfigure}
%	\caption{\label{fig:rirexampleF} \sl %{\bf Same remark as for Fig.~\ref{fig:efr2} }
%		Comparaison de $r_{IR}$ entre les données et les simulations pour trois {\sc Geant}4  listes physiques de l'\'energies 2 (a) et 10 (b) GeV de particule primordiale.}
%\end{figure}

%\begin{figure}
%	\centering
%	\protect\includegraphics[width=0.5\textwidth]{ECAL/plots/r-ir-graph.pdf}
%	\caption{\label{fig:irrgraphF} \sl Radius lateral moyen de la région d'interaction pour les données et les simulations  pour trois listes physiques \geant\ comme une fonction de l'énergie du faisceau (2 \, GeV à 10 \, GeV).}
%\end{figure}

Un résultat central de l'analyse est le nombre de traces secondaires ($N_ {tracks}$). %et les observables en fonction de leurs propriétés.
Les distributions $N_ {tracks}$ sont présentées dans la Fig.~\ref{fig:NtrackF} pour  les données et les trois modèles de GEANT4 pour les énergies des pions primaires de 2 et 10 GeV. 

La valeur moyenne du nombre de traces est présentée en Fig. 1.9 en fonction de l'énergie des pions primaires. Les modèles de GEANT4 sont en bon accord avec les données à 2 et 10 GeV. Par contre ils sous-estiment le nombre de traces d'environ 7\% pour ces deux valeurs.   

%Les trois listes de physique, présentées dans la Fig.~\ref{fig:fulltrackgraphF}, sous-estiment le nombre de traces secondaires de 7\% en moyenne inférieures à 10\,GeV et sont en accord avec les données à 10\,GeV.
\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/ntracks-2.pdf}
		\caption{\label{fig:tr2F} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/ntracks-10.pdf}
		\caption{\label{fig:tr10F} }
	\end{subfigure}
	\caption{\label{fig:NtrackF} \sl Comparaison de $N_{tracks}$ entre les données et les simulations pour trois modèles de simulation de  {\sc Geant}4. L'énergie du pion primaire est de 2 GeV (a) et 10 GeV (b).}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/ntracks-graph.pdf}
		\caption{\label{fig:tracksgraphF} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=.90\linewidth]{ECAL/plots/ntracks-graph-delta.pdf}
		\caption{\label{fig:dtracksgraphF}}
	\end{subfigure}
	\caption{\label{fig:fulltrackgraphF} \sl Nombre moyen de traces trouvées pour les données et les simulations  pour trois listes physiques \geant\ en fonction de l'énergie du faisceau (2\,GeV à 10\,GeV). }
\end{figure}


%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{Les quarks top et bottom à l'ILC}

La masse du quark top est comparable à la valeur du vide électrofaible et elle est beaucoup plus grande que les masses de toutes les autres particules connues aujourd'hui et notamment de celles des bosons de la force électrofaible.
\c C'est pourquoi le quark top  joue un rôle particulier dans de nombreux modèles de physique au-delà du modèle standard.

Des mesures précises des couplages des quarks lourds sont donc des pistes prometteuses pour la recherche indirecte de nouvelles particules et la discrimination entre différentes théories.

Cette section porte sur la production électrofaible des paires de quarks top et bottom.

Les paires de fermions $f$ sont produites au vertex $f\bar{f}X$, où $X$ représente des bosons vectoriels neutres, le photon ou le boson $Z^0$. Le courant au $f\bar{f}X$ vertex peut être exprimé comme suit:
\begin{equation}
\Gamma^{f\bar{f}X}_\mu (k^2,q,\bar{q}) = ie\{ \gamma_\mu (F^X_{1V}(k^2) + \gamma^5 F^X_{1A}(k^2)) - \frac{\sigma_{\mu\nu}(q-\bar{q})^\nu}{2m_f}(iF^X_{2V}(k^2) + \gamma^5 F^X_{2A}(k^2)) \},
\end{equation}
où $k^2= (q+\bar{q})^2$ est la quadri-impulsion au carré du boson du vecteur échangé, $q$ et $\bar{q} $ sont les quadri-impulsions du fermion $f$ et de l'antifermion $\bar{f}$ et $m_f$ est la masse des deux,  $\gamma_\mu$ et $\gamma_5$ sont les matrices de Dirac, et $\sigma_{\mu\nu} = i/2(\gamma_\mu\gamma_\nu - \gamma_\nu\gamma_\mu)$.

$F$ sont des facteurs de forme, qui contiennent les corrections quantiques du vertex. Au niveau Born les $F$ prennent les valeurs suivantes:  
%Les valeurs de \sm\ du facteurs de forme sont les suivantes:
\begin{equation}
F^{f\gamma}_{1V} = Q^{f}, \ F^{f\gamma}_{1A} = 0, \ F^{fZ}_{1V} = \frac{I^f - 2Q^f\sin^2\theta_W}{2\cos\theta_W\sin\theta_W}, \ F^{fZ}_{1A} = - \frac{I^f}{2\cos\theta_W\sin\theta_W},
\label{formula:SMformFactors_3F}
\end{equation}
et tous les $F_2$ sont 0. Dans l'équation~\ref{formula:SMformFactors_3F} $I^f$ est  l'isospin faible, $I^t = 1/2$ pour le quark top et $I^b = -1/2$ pour le quark bottom  et $Q^f$ est la charge electrique, $Q^t = 2/3$ et $Q^b = -1/3$.


Le facteurs de forme sont liés aux couplages des fermions pour des hélicités droite et gauche au boson de $Z^0$, $g_L = F^Z_{1V} - F^Z_{1A}$  et $g_R = F^Z_{1V} + F^Z_{1A}$.
Les résultats obtenus dans cette these sont exprimés en termes de $g_L$ et $g_R$.  
%The form factors are related to fermion couplings with left and right-handed helicity to $Z^0$ boson:
%La définition suivante des couplages gauches et droites $Z^0b\bar{b}$ est utilisée tout au long de la thèse: 
\begin{equation}
%g_L^Z = (F_{1V}^Z - F_{1A}^Z), \  g_R^Z = F_{1V}^Z + F_{1A}^Z, 
g_L^Z = \frac{I^f - Q^f\sin^2\theta_W}{\sin\theta_W\cos\theta_W}, \  g_R^Z = -\frac{Q^f\sin^2\theta_W}{\sin\theta_W\cos\theta_W}.
\label{formula:EWcouplings_3F}
\end{equation}

L'observable clé de la thèse est la section efficace différentielle par rapport de l'angle polaire $\theta$ de diffusion de pair des fermions. La section efficace peut être definie en fonction de la polarisation $I=L, R$  des electrons incidents.    
%L'expression clé pour les études est la section efficace différentielle de $f\bar{f}$ production pour la polarisation du faisceau d'électrons $I=L,R$, exprimée par les facteurs de forme définis:

\begin{multline}
% \frac{\pi\alpha^2 N_c\beta}{s}
\label{formula:DiffSigma_3F}
\frac{d\sigma^I}{d\cos\theta} = \frac{3}{4} \mathcal{A} N_c \beta[ (1+\cos^2\theta) [(\mF_{1V}+\mF_{2V})^2+(\beta \mF_{1A})^2] - \\-4 \cos\theta (\mF_{1V}+\mF_{2V})\beta \mF_{1A} +\\+ \sin^2\theta [\gamma ^{-2} (\mF_{1V} +\gamma^2 \mF_{2V})^2] ]
\end{multline}
Les facteurs $\mathcal{F}$ sont une rédéfinition des facteurs de forme $F$ selon la référence~\cite{bib:Schmidt}, $\mathcal{A} = 4\pi\alpha^2/3s$ où $\alpha$ est le carré du couplage électromagnétique et $N_c$ est le nombre de couleurs des fermions (i.e. 3 pour les  quarks). Finalement, $\beta$ et $\gamma$ sont la vitesse et le facteur de Lorentz du fermion produit, respectivement.

%Les mesures de $sin^2\theta_W$ avec un processus de $e^+e^- \to b \bar{b}$ aux les expériences du collisionneurs LEP et SLC, ont révélé une déviation avec la prédiction de la \sm~\cite{bib:AfbSMFit}.
Les mesures de $\sin^2\theta_W$ par SLD en utilisant l'asymétrie gauche-droite et au LEP en utilisant l'asymétrie avant-arrière dans le processus $e^+e^-\to b\bar{b}$ sont contradictoires entre elles et en désaccord avec la prédiction du modèle standard.  
De nombreuses théories au delà du modèle standard prédisent notamment des modifications de la production électro-faible des paires des quarks lourds par rapport du modèle standard.
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{Reconstruction de la charge du quark bottom}
La reconstruction de la section efficace différentielle de quarks lourds nécessite la mesure de la charge du quark bottom.
A cette fin, cette thèse exploitent deux méthodes complémentaires:
\begin{itemize}
	\item \textbf{Charge de vertex} qui est la somme de toutes les charges reconstruites associées à la desintégration d'un $b$;
	\item \textbf{Charge du méson K} qui est la charge des mésons $K$ associés à la désintégration d'un $b$.
\end{itemize}

%<<<<<<< HEAD
Dans leurs versions actuelles les algorithmes de vertexing ignorent une ou plusieurs particules produites lors de la désintégration des $b$. La qualité de la reconstruction des vertex de desintégration $b$ est définie par l'observable de pureté, definie comme le nombre de charges correctes divis\'e par le nombre total de charges.
Cette thèse propose un algorithme pour récuperer les traces ignorées. Cet algorithme mène à une amélioration significative de la pureté comme le démontre la Fig.~\ref{fig:RecoveryPurityComparison_3F}.%  Les graphiques de la pureté de la charge de vertex avant et apr\'es d'application de la procedure sont représentés dans la Fig.~\ref{fig:RecoveryPurityComparison_3F}.

Le volume gazeux de la TPC permet de mesurer le dépôt d'énergie par longueur de trace, $dE/dx$. La valeur  $dE/dx$ varie en fonction du type et de la vitesse d'une particule et est donc un moyen pour l'identification des particules.  Après avoir corrigé le $dE/dx$ d'effets de dépendance angulaire, les kaons issus de la desintégration des  $b$ peuvent être identifiés avec 97\% de pureté et 87\% d'efficacité.
Les spectres $dE/dx$ en fonction de l'impulsion des particules pour trois types de hadrons apr\'es et avant  la correction angulaire sont représentés dans la Fig.~\ref{fig:dEdxBefore_3F}.
%=======
%On a constaté que les algorithmes de vertexing peuvent manquer une ou plusieurs particules de la desintégration des hadrons de $b$. Cela  diminuit evidemment sur la bonne reconstruction de  la charge de vertex.
%La procédure de récupération de toutes les traces issues de la desintégration des hadrons de $b$  améliore la reconstruction de la charge de vertex en ajoutant les particules de b-hadron ratées aux vertices mesurés à l'aide d'un ensemble d'observables reconstruits.

%L'identification kaon est possible en utilisant les informations TPC $dE/dx$. Après avoir égalisé le $dE/dx$ dans le spectre angulaire, les kaons des sommets des b-hadrons peuvent être identifiés avec 97\% de pureté et 87\% d'efficacité.

%Les graphiques de la pureté de la charge de vertex et le $dE/dx$ en fonction de l'impulsion des particules pour hadrons différents sont représentés dans la Fig.~\ref{fig:RecoveryPurityComparison_3F} et la Fig.~\ref{fig:dEdxBefore_3F}, respectivement.
%>>>>>>> 8e36eba08c2388bfd3f0081d6e8eb96636cb3e72

\begin{figure}
	{\centering
		\protect\includegraphics[width=0.95\textwidth]{ILD/plots/recovery-purity-comparison.pdf}
		\caption{\sl Pureté de la charge en fonction de b-tag - une probabilite pour un jet de provenir d'un quark $b$, l'impulsion du $b$ reconstruit, $N_ {rec}$ et l'angle polaire $|\cos\theta|$ avant et après l'algorithme de récupération de vertex. 
		}
		\label{fig:RecoveryPurityComparison_3F}
	}
\end{figure}

\begin{figure}
	{\centering
		\protect\includegraphics[clip, trim=8cm 18.5cm 7cm 4cm,width=0.95\textwidth]{ILD/plots/dedx-before.png}
		\caption{\sl Le dépôt d'énergie par longueur de trace $dE/dx$ en fonction de l'impulsion des particules, l'angle polaire des particules $|\cos\theta|$ pour pions, kaons et protons. Deux lignes grises séparent la région avec une concentration maximale de kaons.
		}
		\label{fig:dEdxBefore_3F}
	}
\end{figure}

\begin{figure}
	{\centering
		\protect\includegraphics[clip, trim=8cm 18.5cm 7cm 4cm, width=0.95\textwidth]{ILD/plots/dedx-after.png}
		\caption{\sl Le dépôt d'énergie par longueur de trace $dE/dx$ en fonction de l'impulsion des particules, l'angle polaire des particules $|\cos\theta|$ pour pions, kaons et protons. apr\'es l'application de la correction angulaire.  Deux lignes grises séparent la région avec une concentration maximale de kaons.
		}
		\label{fig:dEdxAfter_3F}
	}
\end{figure}


%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
\newpage
\subsection*{Reconstruction de l'angle polaire des quark top et bottom}
L’\'etude du quark top suppose une \'energie dans le centre de masse de $\sqrt{s} = 500$\,GeV et une luminosit\'e int\'egr\'ee de $500$\ifb. 
Le quark top désintègre en quark bottom et boson $W$. Le désint\'egration du boson $W$ définit trois topologies pour le processus $e^+e^-\to t\bar{t}$:
\begin{itemize}
	\item le canal leptonique $ t\bar{t} \to b\bar{b} l^+ \nu l^- \bar{\nu}$;
	\item le canal semi-leptonique $ t\bar{t} \to b\bar{b} l \nu q \bar{q}'$;
	\item le canal hadronique $ t\bar{t} \to b\bar{b} q \bar{q}' q \bar{q}'$.
\end{itemize}
 L'analyse précédente~\cite{bib:ILCTOP} a utilisé la charge du lepton $W^\pm$ pour reconstruire  l'asymétrie avant-arrière $A_ {FB}$, définie comme le nombre d'événements émis à l'avant moins le nombre d'événements émis à l'arrière divisé par le nombre total.
 %la différence normalisé entre les nombres d’\'ev\'enements dans les h\'emisph\`eres du d\'etecteur par rapport \'a l'angle polaire.  
Cette observable est sensible aux facteur de forme axial $F_{1A}^{Z/\gamma}$.


Dans un premier temps, les nouvelles méthodes de reconstruction de la charge du quark $b$ ont été appliquées dans le canal semi-leptonique du quark top pour améliorer l'efficacit\'e de la reconstruction de la charge du quark top.
Le résultat après l'application de toutes les combinaisons de paires possibles de la charge de vertex, de la charge de kaon et de la charge de $W^\pm$ lepton à la reconstruction de l'angle polaire supérieur illustrée dans la Fig.~\ref {fig:TopAsymmetryChi_3F}.

%<<<<<<< HEAD
Cette méthode permet de reconstituer l'asymétrie avant-arrière du quark top avec $A_ {FB}^{rec} / A^{gen}_{FB} = 94\%$. L'efficacité finale de la selection est de 38,6\%, ce qui améliore le résultat précédent~\cite{bib:ILCTOP} par 25\%.
%=======
%Cette méthode permet de reconstruire l'asymétrie avant-arriere $A_{FB}$ aussi bon que $A_ {FB}^{rec} / A^{gen}_{FB} = 94\%$ avec l'efficacité finale de 38,6\%, ce qui améliore le résultat précédent~\cite {bib:ILCTOP} par 25\%.
%>>>>>>> 8e36eba08c2388bfd3f0081d6e8eb96636cb3e72

La méthode la plus utilisée est la combinaison de la charge de vertex avec la charge $W^\pm$ lepton car le $ W^\pm$ lepton doit être reconstruit dans chaque événement sélectionné.

\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\protect\includegraphics[width=0.95\textwidth]{ILD/plots/top-asymmetry-lepton.pdf}
		\caption{\label{fig:TopAsymmetryChi_a_3F} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=0.95\textwidth]{ILD/plots/top-methods-lepton.pdf}
		\caption{\label{fig:TopAsymmetryChi_b_3F} }
	\end{subfigure}
	\caption{\sl Distribition de l'angle polaire génére par rapport à l'angle polaire reconstruit (a) du quark top en utilisant toutes les combinaisons possibles de signature de charge, dont la répartition est donnée en (b).}
	\label{fig:TopAsymmetryChi_3F}
\end{figure}

%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%En suit, on peut appliquer les nouvelles methodes pour extraction des couplages \'electrofaibles du quark $b$. 
Pour le canal $e^+e^-\to b\bar{b}$ on utilise seulement la détermination de la charge du quark $b$ pour la reconstruction de l'angle polaire.
La distribution de l'angle polaire reconstruit du quark $b$ à $\sqrt{s} = 250$\,GeV utilisant une combinaison de signatures des charges des kaons et du vertex est montrée sur la Fig. ~\ref{fig:BAsymmetryFinal_3F}. 
Une luminosité intégrée $\mathcal{L}_I=250$\,fb$^{-1}$ est supposée pour chaque polarisation du faisceau.

%\subsection*{Reconstruction de l'angle polaire du quark bottom et top}

\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\protect\includegraphics[width=0.95\textwidth]{ILD/plots/basymmetry-final-left.pdf}
		\llap{\shortstack{%
				\protect\includegraphics[clip, trim=0cm 0cm 1.8cm 1.7cm, scale=.14]{ILD/plots/zoom-final.pdf}\\
				\rule{0ex}{0.38in}%
			}
			\rule{1.8in}{0ex}}
		\caption{\label{fig:BAsymmetryFinal_a_3F} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=0.95\textwidth]{ILD/plots/basymmetry-final-right.pdf}
		\caption{\label{fig:BAsymmetryFinal_b_3F} }
	\end{subfigure}
	\caption{\sl Distribution de l'angle polaire des quarks b générée comparées aux distributions de l'angle polaire des quarks b reconstruit pour la configuration $P_{e}-=-1, P_{e^+}=+1$ (a) et $P_{e}-=+1, P_{e^+}=-1$(b) les processus de fond sont superposés  et indiqués en rouge.}
	\label{fig:BAsymmetryFinal_3F}
\end{figure}

Le spectre final est obtenu par une correction supplémentaire qui se sert des mesures contradictoires des charges sans faire appel à l'information du générateur.  % En utilisant les puretés mesurées, le spectre reconstruit est corrigé à l'aide d'une procédure basée sur les données.
Les distributions corrigées sont ajustées par $S(1+\cos^2\theta) + A\cos\theta$ conformément à  Eq.~\ref{formula:DiffSigma_3F}. Les paramètres $S$ et $A$ sont donc reliés aux constantes de couplage. 
%La précision extraite sur les paramètres $S$ et $A$ est extrapolée à la polarisation réaliste $\pm 0.8, \mp 0.3$ et à le répartition de la luminosité du programme de physique de l'ILC.
Comme on peut le voir dans la Fig.~\ref{fig:BAsymmetryFinal_3F}, la contribution des processus de fond, comme par exemple la production d'une paire de bosons est faible.

\begin{figure}
	\centering
	\begin{subfigure}{0.5\textwidth}
		\protect\includegraphics[width=0.99\textwidth]{ILD/plots/lep-result-zoom.pdf}
		\caption{\label{fig:LEPILCResult_a_3F} }
	\end{subfigure}% 
	\begin{subfigure}{0.5\textwidth}
		\centering
		\protect\includegraphics[width=0.99\textwidth]{ILD/plots/ilc-result.pdf}
		\caption{\label{fig:LEPILCResult_b_3F} }
	\end{subfigure}
	\caption{\sl Les régions de $\pm 1\,\sigma$ sur les couplages $Z^0b\bar{b}$ définies par l'asymétrie avant-arrière et les mesures des sections efficaces totales à LEP (a) et à l'ILC via l'ajustement de la section différentielle (b). Les lignes directrices montrent les valeurs de la \sm.
		Les valeurs centrales de la projection de la precision de  l'ILC est déplacé vers les valeurs de la \sm.
	}
	\label{fig:LEPILCResult_3F}
\end{figure}

Les précisions relatives sur les couplages $Z^0 b\bar{b}$, $g_L^Z$ et $g_R^Z$, pour les mesures LEP~I et pour les performances attendues à l'ILC sont affichées dans la Fig.~\ref{fig:LEPILCResult_3F}. 
La précision de l'ILC sur le couplage $g_R^Z$ est suffisante pour confirmer ou rejeter complètement l'anomalie observée à LEP dans le processus $e^+e^-\to b\bar{b}$.



\subsection*{Conclusions}

Cette thèse présente de nouvelles méthodes et études développées pour l'analyse de données qui seront enregistrées avec les détecteurs de l'ILC. 
Ces détecteurs sont conçus pour l'application d'algorithmes, qui améliorent la reconstruction des états finaux des collisions $e^+e^-$ en utilisant les informations des calorimètres hautement granulaires.
En plus ces détecteurs sont également conçus pour une mesure très précise des vertex secondaires.

Le prototype du calorim\`etre \'electromagn\'etique hautement granulaire a été construit et testé par la collaboration CALICE.
Dans cette thèse, un algorithme de reconstruction des traces a été développé permettant d'étudier pour la première fois des traces secondaires issues des interactions hadroniques dans le prototype SiW-ECAL.
%La simulation de SiW-ECAL a été comparée aux données en utilisant les nouvelles observables de l'algorithme de recherche de traces.
Les données enregistrées avec ce prototype lors des campagnes de test en faisceau sont comparées avec des prédictions des modèles des gerbes hadroniques proposés par le logiciel GEANT4. L'algorithme donne accès à de nouvelles observables représentées comme le nombre de traces par interaction. 


Tous les modèles de simulation testés montrent une bonne performance en termes de nouvelles observables à l'exception de 10-15\% différence dans les observables de la zone d'interaction.

Dans cette thèse, les distributions de l'angle polaire des quarks top et bottom sont obtenues à l'aide de la charge du quark b.  
Les méthodes développées sont appliquées aux deux canaux, $e^+ e^- \to t\bar{t}$ et $e^+ e^- \to b\bar{b}$ à $\sqrt {s} = 500$\,GeV et 250\,GeV, respectivement.

La thèse propose des méthodes pour la determination de la charge du quark $b$ avec une haute pureté: la somme de toutes les charges reconstruites, qui sont associées au vertex de desintégration des $b$ et la charge des kaons trouvés dans les produits de la desintégration des $b$. 
Cela permet de reconstruire précisement l'angle polaire du quark $b$ et d'en extraire les couplages électrofaibles du quark $b$ au boson de $Z^0$. % permet de corriger la distribution  de l'angle polaire pour la contamination résiduelle.
%En conséquence, l'angle polaire du quark bottom reconstruit est utilisable pour l'extraction des couplages  et des facteurs de forme électrofaibles du quark bottom.
La précision previsible à l'ILC sur le couplage $g_R$ est 5 fois meilleure que pour LEP. L'anomalie LEP sera soit donc confirmée, soit définitivement écartée.




==> Introduction.tex <==
%\section{Introduction}

The \sm\ of particle physics provides a unified description of electromagnetic, weak and strong forces. It has been developed by a wide scientific community in the middle of 20th century and has been confirmed by numerous experiments. 

The latest triumph of the \sm\ is the discovery of the Higgs boson at the Large Hadron Collider (LHC) experiments at CERN, CMS~\cite{bib:HiggsCms} and ATLAS~\cite{bib:HiggsAtlas}, in July 2012.
%TOP?
Another great success of the \sm\ is the discovery of the top quark by TeVatron collaborations in 1995. Top quark is the heaviest elementary particle found, which plays an important role in the \sm\ and cosmology. 
So far, the Higgs boson and the top quark were precisely studied in hadron collisions by the TeVatron and LHC experiments. Therefore, a precise measurement of electroweak coupling constants of the particles is left for the future experiments.

Despite its success, the \sm\ leaves many experimental and theoretical phenomena without a definite answer. 
%Therefore many \bsm (BSM) theories have been developed. 
Indirect evidences of New Physics call for new high energy frontier colliders.

The International Linear Collider \cite{bib:ILC} (ILC) is a high energy electron-positron collider project aimed at precision measurements and New Physics searches. 
The ILC is designed to operate at the center-of-mass energy $\sqrt{s}=500$\gev, which is ideal for studies of electroweak interactions of the top quark. 
Well known leptonic initial state at the ILC allows clean, model-independent analysis of \sm\ processes as well as for BSM searches. 
%CALO?

The highly granular calorimeters of ILC detectors allow accurate particle separation required by Particle Flow reconstruction algorithms.

This thesis consists of three parts: the theoretical background and ILC description, data analysis of hadronic interactions in a highly granular calorimeter prototype and an update of the top quark production analysis in the ILC environment.
The final part describes the new results on the electroweak couplings of the b-quark at the ILC.

Part~\ref{PARTI} gives the necessary background for the thesis subject. A brief introduction into the theoretical framework of the \sm\ provided in Sec.~\ref{sec:SM}, and the description of the ILC project is described in Sec.~\ref{sec:ILC}.

Part~\ref{PARTII} of the thesis concentrates on the analysis of the beam test data recorded with the CALICE Silicon-Tungsten Electromagnetic Calorimeter (\ecal) physics prototype. The granularity of this device allows disentangling fine details of the hadronic interaction events. Sections~\ref{sec:Passage}, \ref{sec:ecalintro} provide an introduction to the topic. Section~\ref{sec:track} describes the reconstruction of the secondary tracks from the $\pi^-$ interaction. 
In Sec.~\ref{sec:results} one finds the data-simulation comparison using new variables from the developed track-finding algorithm.

Part~\ref{PARTIII} unites several studies  of the $e^+e^- \to t\bar{t}$ and $e^+e^- \to b\bar{b}$ channels at the ILC.
% performed using a full simulation of the ILD experiment. 
Chapter~\ref{sec:Phenomenology} introduces a common theoretical framework of the heavy quark production. Section~\ref{sec:JetChargeReconstruction} describes the methods of the b-quark charge measurement. In Chapters~\ref{sec:TopProduction} and~\ref{sec:BProduction} one finds the application of the b-quark charge technique to the top and bottom quark production studies at the ILC, respectively. New studies of the expected precision on the bottom quark couplings at the ILC are provided in Sec.~\ref{sec:NewResults}. 













==> intro/corrections.tex <==
In QCD there are Yang-Mills with local color group SU(3) - color.
Coupled to six dirac fields (quarks) with different masses and flavours. 
Vector fields of gluons.
QCD Lagrangian is




For NRQCD
ΛQCD ≪νNR ≪m, where νNR is ultraviolet cut-off of theory
in NRQCD \QQbar pair cannot be created and usage of Pauli spinors is enough.

NRQCD is rogorous and reproduces QCD up to some order of alpha_s, v


Lagrangian NRQCD can be written in the following way...
Lorenz invariance leads to c2 = c4 = 1, cS = 2cF − 1 [19, 22–26].
The matching coefficients may be calculated in perturbation theory.


Since several scales remain dynamical in NRQCD, it is not possible to give a homogeneous power counting for each operator without extra assumptions, i.e., the power counting in v is not unambiguous. To obtain a better defined power counting one should go to EFTs of lower energy. It should be noticed that the importance of a given operator for a practical calculation does not depend only on its size, but also on the leading power of αs of the corresponding matching coefficient.


\subsection{Lower energy EFTs}
pNRQCD and vNRQCD
For detailed recent reviews on effective field theories for heavy quarkonium we refer the reader to [10] and [11], which are mainly devoted to pNRQCD and vNRQCD respectively.



What we want to point out here is that in all these EFTs objects like potentials show up. For short range (or weakly coupled) quarkonia the potentials may be built order by order in perturbation theory. At higher order the pure potential picture breaks down and the interaction of the heavy quark fields with the low-energy gluons has to be taken into account


The potential picture that emerges from these EFTs is quite different from the one of traditional potential models and superior. Not only the potential is derived from QCD, but higher-order corrections can be systematically included without being plagued by divergences or ad hoc cut-offs; these are ab- sorbed in the renormalization procedure of the EFT. Nevertheless, traditional potential models, which so much have contributed to the early understanding of the heavy quarkonium properties, may be still useful and will often appear in the report. First, a potential model can be seen, in absence of competitive lattice data, as a specific ansatz on the form of the low-energy QCD dynamics encoded in the potential defined by an EFT. Second, potential models still provide the only available tool to describe physical systems for which a suitable EFT has not been built yet. This is, for instance, the case of systems coupled to open flavour channels.


\section{potantials}
[T + V ]Ψ = EΨ
We lump into these approaches the Bethe–Salpeter equation (e.g., Ref. [182, 184]) and quasi-potential approaches (e.g., Ref. [173]).

Different approaches have been used for the kinetic energy term ranging from the non-relativistic Schro ̈dinger equation to relativistic kinetic energy [171,179,189]
in the spinless Salpeter equation.

The quark–antiquark potential is typically motivated by the properties expected from QCD [48,128–134] and while there are differences, most recent potentials show strong similarities. It is worth pointing out that in the early days of quarkonium spectroscopy this was not obvious and much effort was expended in fitting different functional forms of the potential to the observed quarkonium masses. In the end, the shape of the potentials converged to a form that one might expect from the asymptotic limits of QCD and which has been qualitatively verified by Lattice QCD calculations [135] of the expression of the potentials obtained in the Wilson loop [128–134] and in the EFT [48] approach. This is a great success of quarkonium phenomenology.


To derive the quarkonium potential we start with QCD where the gluons couple to quarks and to each other. The quark–gluon interaction is similar to the electron–photon interaction in quantum electrodynamics with the Born term for the qq or qq ̄ interaction at short distance being the familiar 1/r form. In contrast with QED the gluon self-coupling results in a slow decrease of the effective coupling strength at short distance. In terms of the Fourier conjugate momentum the lowest order QCD corrections to αs = gs2/4π can be parametrized as
αs(Q2) = 12π (3.26) (33 − 2nf ) ln(Q2/Λ2)

where nf is the number of Fermion flavours with mass below Q, and Λ ∼ ΛQCD is the characteristic scale of QCD measured to be ∼ 200 MeV. At short distances one-gluon-exchange leads to the Coulomb like potential
V (r) = −4 αs(r)

for a qq ̄ pair bound in a colour singlet where the factor of 4/3 arises from the SU(3) colour factors. At short distances one-gluon-exchange becomes weaker than a simple Coulomb interaction.

At momentum scales smaller than ΛQCD which corresponds to a distance of roughly 1 fm, αs blows up and one-gluon-exchange is no longer a good representation of the qq ̄ potential. The qualitative picture is that the chromoelectric lines of force bunch together into a flux tube which leads to a distance- independent force or a potential
V (r) = σr. (3.28) This has been validated by Lattice QCD calculations. Phenomenologically, every recent model which
we will consider has found σ ∼ 0.18 GeV2.

Numerous variations of the resulting Coulomb plus linear potential exist in the literature. Some of the better known ones are the Cornell potential [170], Richardson’s potential [190], and the Buchmu ̈ller Tye potential [191]. Overall, the spin-independent features of quarkonium spectroscopy are well de- scribed by the potentials just described.


Let us also mention that heavy quark mass corrections to the (static) central (spin and velocity
independent) potential exist, although they have not yet been taken into account in potential models
applications so far. They correspond to V (1,0) , V (2,0) and V (1,1) in Section 2.3.2. Their expressions in rrr
perturbation theory are known [48, 68]. Part of V (2,0) and V (1,1) was included in the phenomenological rr
application to the spectrum in Refs. [128, 129, 135, 185].


Simply put, one can obtain the form of the spin dependent interaction by Fourier transforming the on-shell qq ̄ scattering amplitude:
M = [u ̄(p′f )Γu(p′i)] V (Q2) [u ̄(pf )Γu(pi)] (3.29)
where the Γ matrices give the Lorentz structure of the interaction and V (Q2) is the Fourier transform of the spin-independent potential. For example, for a Lorentz-vector interaction Γ = γμ and for a Lorentz- scalar interaction Γ = I. In principle other forms are possible with each giving rise to characteristic spin-dependent interactions. These can be found by expanding the scattering amplitude to order (v/c)2 which corresponds to an expansion in inverse powers of quark masses. In the early years of quarko- nium phenomenology they were all tried and it was found that the Lorentz-vector one-gluon-exchange plus Lorentz scalar linear confining potential gave the best agreement with experiment 23. Note that the form of the full QCD potential at order 1/m2 [48, 128, 130–133] has now been obtained in the EFT (cf. Section 2.3.2), and while the spin-dependent nonperturbative potential may correspond to a scalar interaction in the language used above, the velocity-dependent potentials do not fit such a picture. The effective kernel is thus not a simple scalar, precisely the dependence both on the momentum and on the Lorentz structure is more involved than a pure convolution (i.e., only depending on the momentum trans- fer) scalar structure [48, 134, 138, 186]. However, the spin dependency is well approximated by a scalar interaction for phenomenological applications. The QCD spin-dependent potentials are explicitly given in Section 2.3.2. A complete calculation of the spin structure of the spectrum using the full expression given in Section 2.3.2 does not yet exist.

To lowest order in (v/c)2 the Lorentz-vector one-gluon-exchange gives rise to terms familiar from
one-photon exchange in atomic physics. The colour contact interaction, which in the language of Sec-
tion 2.3.2 corresponds to taking V (1,1)(r) at leading order in perturbation theory, S2
Hcont = 32π αs(r) S · S δ3(r) (3.30) qq ̄ 9mqmq ̄qq ̄
q q ̄ 3 m q m q ̄ r 3 r 2 q q ̄
S12
H t e n = 4 α s ( r ) 1 􏰋 3 S q · r S q ̄ · r − S · S 􏰌 ( 3 . 3 1 )
CHAPTER 3
  gives rise to, for example the J/ψ − ηc splitting. The colour tensor interaction, which in the language of Section 2.3.2 corresponds to taking V (1,1)(r) at leading order in perturbation theory,
    contributes to splitting of L ̸= 0 spin triplet multiplets like the χcJ and χbJ multiplets. The final spin dependent term is the spin orbit interaction which has two contributions. The first piece arises from the colour-magnetic one-gluon-exchange while the second piece is the Thomas precession term which is a relativistic effect for an object with spin moving in a central potential
Hs.o. = Hs.o.(cm) + Hs.o.(tp). qq ̄ qq ̄ qq ̄
The colour magnetic piece arising from one-gluon exchange is given by:
Hs.o.(cm)=4αs(r)􏰉 Sq + Sq ̄ +Sq +Sq ̄􏰊·L


\section{2.2}


There it was shown in particular that: a Schrödinger picture of the quarkonium dynamics emerges at some order in the velocity expansion in non-relativistic EFTs of QCD; 

how to express the potential in terms of well defined quantities to be computed in QCD either in perturbation theory or with lattice QCD; 

the Schrödinger picture fails at some point; 

what are the first non-potential corrections and how to compute them. 

Moreover it was emphasized that ground state quarkonium (Y(1S), J/psi, Bc) may be computed (to a large extent, nonperturbative corrections are small) in perturbation theory, hence precision physics is possible for these quantitites (in particular one may extract the b,c masses, compute the strong coupling, the hfs splittings, M1 transitions widths, leptonic widths, total widths). 

While excited states are inherently nonperturbative and require lattice input (for the potentials). 
However most of the lattice potentials (spin dependent and spin indipendent) have indeed been computed.

Non-relativistic effective field theories follow from QCD by systematically integrating out the high energy scales and replacing QCD by suitable expansions. 

The first EFT is NRQCD that follows from QCD by integrating out modes associated with the heavy quark mass scale m. 

The ultimate EFT, where a Schrödinger picture emerges, is potetial NRQCD (pNRQCD), which follows from QCD by integrating out all energy scales above mv^2 (say at least m and mv), where v is the quark-antiquark relative velocity. 

Looking at production processes one may want to integrate first out the transverse momentum p_T, before proceeding with NRQCD. This introduces another EFT.

The description of section 2.2 seems to transmit the idea that we are still stuck with the Buchmüller-Tye or the Godfrey-Isgur models. But, as I said, a lot has been done from the eighties to make quarkonium physics a rigorous application of QCD. And much precision physics has been extracted in this way. The sentence "The quarkonium spectrocopy is important for potential models and lattice calculations." does not reflect at all this reality and diminuishes without reasons the actual relevance of your work.

So, I would rewrite section 2.2 in the modern spirit of non-relativistic EFTs. This would also be beneficial to introduce properly NRQCD, which plays such a big role in the rest of the thesis. It is surprising in fact that in the thesis the words "effective field theory" are never used. But NRQCD is an EFT and so is the theory underlayng the Schrödinger equation, once properly derived from QCD.






\section{2.3}

\section{8.1}










==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash aleph} & \aleph & \texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal \\
\texttt{\textbackslash lthree} & \lthree & \texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash muon} & \muon \\
\texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb \\
\texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pizs} & \pizs & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson \\
\texttt{\textbackslash rhoz} & \rhoz & \texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom \\
\texttt{\textbackslash rhopm} & \rhopm & \texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb \\
\texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp \\
\texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp \\
\texttt{\textbackslash etaz} & \etaz & \texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz \\
\texttt{\textbackslash omegaz} & \omegaz &  \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash DorDbar} & \DorDbar \\
\texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz \\
\texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash Ds} & \Ds \\
\texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm \\
\texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp \\
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb \\
\texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp \\
\texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Lz} & \Lz \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar & \texttt{\textbackslash Lambdares} & \Lambdares \\
\texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar \\
\texttt{\textbackslash Sigmaresbarz} & \Sigmaresbarz & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Lc} & \Lc \\
\texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz \\
\texttt{\textbackslash Xibm} & \Xibm & \texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz \\
\texttt{\textbackslash Xibbarp} & \Xibbarp & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb & \texttt{\textbackslash Vuds} & \Vuds \\
\texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds & \texttt{\textbackslash Vuss} & \Vuss \\
\texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss & \texttt{\textbackslash Vubs} & \Vubs \\
\texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt \\
\texttt{\textbackslash dpp} & \dpp & \texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> ppbar/4_summary.tex <==
\clearpage
\section{Summary}
\label{sec:summary}

In summary, using an integrated luminosity of 2.0 \invfb collected in 2015 and 2016, 
the prompt \etac production at $\sqs=13$~\tev centre-of-mass energy is measured for the first time. 
The relative prompt production rates of the \etac and \jpsi states in the LHCb fiducial region ($2.0 < y < 4.5$, $6.5 \gevc < \pt < 14.0 \gevc$)
is measured using \tzfit to distinguish prompt production and production in \bquark-decays to be 
\begin{align*}
(\sigma_{\etac}/\sigma_{\jpsi})_{13 \tev}^{6.5 \gevc < p_T < 14.0 \gevc, 2.0<y<4.5}  
	&= \etacPromptRelativeXsec. 
\end{align*}
Using a \tzcut to distinguish prompt and \bquark-decays production as in Run I data analysis, gives the value consistent with the first result.

Using \jpsi prompt production cross-section measurement at \sqs=13~\tev, the \etac prompt production cross section in the LHCb fiducial region is then derived to be 
\begin{align*}
(\sigma_{\etac})_{13 \tev}^{6.5 \gevc < p_T < 14.0 \gevc, 2.0<y<4.5}  
	&= \etacPromptAbsoluteXsec.
\end{align*} 

The \etac inclusive branching fraction from \bquark-hadron decays is measured using the second technique to be:
\begin{align*}
\BR_{\bToEtacX}/\BR_{\bToJpsiX} &= \etacSecondaryRelativeBR 
\end{align*}
and
\begin{align*}
\BR_{\bToEtacX} &= \etacSecondaryAbsoluteBR. 
\end{align*}
The \tzfit gives consistent results.

% The measurement can be further improved by increasing the sample size. 
Using topological triggers, the \jpsi and \etac mass difference is measured. 
The obtained result , 
$\Delta M_{\jpsi , \, \etac} = M_{\jpsi} - M_{\etac} = \etacMassDiff$, 
is consistent with the world average value and is the most precise \etac mass measurement to date.


